Multi-Objective GFlowNets

We study the problem of generating diverse candidates in the context of Multi-Objective Optimization. In many applications of machine learning such as drug discovery and material design, the goal is to generate candidates which simultaneously optimize a set of potentially conflicting objectives. Moreover, these objectives are often imperfect evaluations of some underlying property of interest, making it important to generate diverse candidates to have multiple options for expensive downstream evaluations. We propose Multi-Objective GFlowNets (MOGFNs), a novel method for generating diverse Pareto optimal solutions, based on GFlowNets. We introduce two variants of MOGFNs: MOGFN-PC, which models a family of independent sub-problems defined by a scalarization function, with reward-conditional GFlowNets, and MOGFN-AL, which solves a sequence of sub-problems defined by an acquisition function in an active learning loop. Our experiments on wide variety of synthetic and benchmark tasks demonstrate advantages of the proposed methods in terms of the Pareto performance and importantly, improved candidate diversity, which is the main contribution of this work.

==> tex/background_gfn_alt.tex <==
We briefly summarize preliminaries necessary for the discussion of MOGFNs.  For a more thorough introduction we refer the interested reader to~\cite{gflownet_foundations}.

Assume we are given a directed acyclic graph (DAG) G = (\mathcal{S}, \mathcal{E}).  The elements s \in \mathcal{S} are termed \textit{states} while the edges (s \rightarrow s') \in \mathcal{E} are coined \textit{edges}.  If there exists the edge (s \rightarrow s') \in \mathcal{E} we call s the \textit{parent} of s' and s' the \textit{child} of s.  There exists a unique \textit{starting state} s_0 \in \mathcal{S} which has no parent, as well as a set of \textit{terminal states} \mathcal{X} \subset \mathcal{S} for which it holds that all members of \mathcal{X} have no children.

A sequence of actions \tau = (s_m \rightarrow s_{m+1} \rightarrow \ldots \rightarrow s_n) is called a \textit{trajectory} and is more specifically called a \textit{complete trajectory} if s_m = s_0 and s_n \in \mathcal{X} (i.e., s_n is a terminal state).  The set of all complete trajectories is written as \mathcal{T}.  A \textit{(forward) policy} is a distribution over trajectories in \mathcal{T} and is given by a factorization over states as

P_F(\tau = (s_0 \rightarrow \ldots \rightarrow s_n)) = \prod_{i=0}^{n-1} P_F(s_{i+1} | s_i)

where each P_F(-|s) is a distribution over edges (s \rightarrow s') \in \mathcal{E}.  

Given a non-negative reward function R: \mathcal{X} \rightarrow \mathbb{R}^+ a GFlowNet aims to learn a policy P_F(\tau) such that for each x \in \mathcal{X} the marginal likelihood of sampling a trajectory terminating in x is proportional to its reward R(x).  This property holds true whenever the \textit{flow matching conditions} are satisfied (we again refer the interested reader to~\cite{gflownet_foundations} for a more complete description).

In practice a GFlowNet is learned in a fashion similar to RL by minimizing an objectives such as the \textit{detailed balance}, \textit{subtrajectory balance}, or \textit{trajectory balance} objectives~\cite{gflownet_foundations, trajectory_balance, subtb} over a set of sampled trajectories.  These objectives involve learning the parameters \theta of a forward policy P_F(-|s; \theta) as well as a backward policy P_B(-|s'; \theta) which provides a distribution over parents of a state s'.  They also require learning either a state flow function F_\theta: \mathcal{S} \rightarrow \mathbb{R}^+ or the partition function Z_\theta = \sum_{x \in \mathcal{X}} R(x).  In this paper use the trajectory balance loss which may be written

\begin{equation}
    \mathcal{L}(\tau;\theta) = \left(\log \frac{Z\theta\prod{s\rightarrow s' \in \tau}P_F(s'|s;\theta)}{R(x)\prod_{s\rightarrow s' \in \tau}P_B(s|s';\theta)} \right)^2.
    \label{eq:tb_loss}
\end{equation}

In this work we train GFlowNets off-policy to encourage better exploration, using a sampling policy which is a mix of the learned P_F(\tau) and a uniform distribution over actions over U along with a parameter \delta controlling the degree of mixing.  Finally, we note that a GFlowNet can be made to sample more stringently from the modes of the distribution p(x) = \frac{R(x)}{Z} by exponentiating the reward function by some constant temperature \beta.  We make use of this fact in our construction of prefence-conditional GFlowNets in Section~\ref{sec:4.1}.


==> tex/intro_ai4mat.tex <==
\section{Introduction}
\label{sec:intro}
Decision making in practical applications often involves reasoning about multiple, often conflicting, objectives~\citep{keeney1993decisions}. 
% Consider the task of material design, which we use as an example throughout the paper. 
For instance, in the design of materials for photovoltaic cells, the goal is to generate \emph{novel} candidate materials (molecules) which have high energy-conversion efficiency, stability, ease of synthesizability and robustness to the elements~\cite{luceno2019materials}. These objectives are conflicting -- molecules with high energy-conversion efficiency can be less stable and harder to synthesize -- so there is no single candidate that maximizes all the objectives simultaneously. Such problems fall under the umbrella of \ac{MOO}~\citep[MOO]{ehrgott2005multicriteria,miettinen2012nonlinear}, wherein one is interested in identifying \emph{Pareto-optimal} candidates. The set of Pareto-optimal candidates cover all the best tradeoffs among the objectives, i.e., the Pareto front, where each point on that front corresponds to a different set of weights associated with each of the objectives.

\emph{In-silico} design of materials is typically driven by proxies that only approximate the true objectives. Since these proxies are generally models trained using finite data, there is epistemic uncertainty associated with their predictions. This makes it critical to generate \emph{diverse} candidates to ensure that at least some candidates end up working in downstream evaluations~\citep{jain2022biological}. Generative Flow Networks~\citep[GFlowNets]{bengio2021flow,bengio2021gflownet} are a recently proposed family of probabilistic models which tackle the problem of diverse candidate generation. Contrary to the reward maximization view of reinforcement learning (RL) and Bayesian optimization (BO), GFlowNets generate candidates with probability proportional to the reward. Sampling candidates, as opposed to greedily generating them, implicitly encourages diversity in candidate generation. GFlowNets have shown promising results in single objective problems of molecule generation~\citep{bengio2021flow} and biological sequence design~\citep{jain2022biological}.

In this paper, we study \emph{Multi-Objective GFlowNets} (MOGFNs), extensions of GFlowNets to tackle multi-objective optimization problems. We consider two variants of MOGFNs -- (a) Preference-Conditional GFlowNets (MOGFN-PC) combining Reward-Conditional GFlowNets~\citep{bengio2021gflownet} with Weighted Sum Scalarization~\citep{ehrgott2005multicriteria} and (b) MOGFN-AL an extension of GFlowNet-AL~\citep{jain2022biological} for multi-objective active learning settings. We empirically demonstrate the advantage of these MOGFNs over existing approaches on a wide variety of tasks relevant for material design: the generation of small molecules, as well as the design of DNA Aptamers and fluorescent proteins. Our contributions are the following

\begin{enumerate}[leftmargin=6mm]
    \item[\textbf{C1}] We introduce two new GFlowNet variants for multi-objective optimization: MOGFN-PC and MOGFN-AL.
    \item [\textbf{C2}]  We empirically demonstrate the efficacy of MOGFN-PC in high-dimensional MOO problems. Our work is the first successful empirical validation of Reward-Conditional GFlowNets~\citep{bengio2021gflownet}.
    \item [\textbf{C3}] Through a series of experiments on practically relevant tasks of molecule generation and sequence generation, we demonstrate that MOGFN-PC generates \emph{diverse} Pareto-optimal candidates.
    \item  [\textbf{C4}] In a challenging multi-objective active learning task for protein design, we show that MOGFN-AL results in significant improvements in sample-efficiency. %for generating \emph{diverse} Pareto-optimal candidates. %Our work is the first to leverage \ac{GFlowNets} for mutation-based biological sequence design.
    % \item [\textbf{C5}] We supplement our results with a thorough analysis of all components of MOGFNs to provide insights on choices that affect performance. 
\end{enumerate}


